Human-centered explanation does not fit all: The interplay of sociotechnical, cognitive, and individual factors in the effect AI explanations in algorithmic decision-making

Recent XAI studies have investigated what constitutes a \textit{good} explanation in AI-assisted decision-making. Despite the widely accepted human-friendly properties of explanations, such as contrastive and selective, existing studies have yielded inconsistent findings. To address these gaps, our study focuses on the cognitive dimensions of explanation evaluation, by evaluating six explanations with different contrastive strategies and information selectivity and scrutinizing factors behind their valuation process. Our analysis results find that contrastive explanations are not the most preferable or understandable in general; Rather, different contrastive and selective explanations were appreciated to a different extent based on who they are, when, how, and what to explain -- with different level of cognitive load and engagement and sociotechnical contexts. Given these findings, we call for a nuanced view of explanation strategies, with implications for designing AI interfaces to accommodate individual and contextual differences in AI-assisted decision-making.

==> tables/tab_cog_vars.tex <==
\addtolength{\tabcolsep}{2pt}
\begin{table*}
\caption{Variables in cognitive load, decision styles, and Motivation-Opportunities-Ability (MOA) model}
\label{tab:cog_vars}
\begin{NiceTabular}[t]{@{}p{2cm}ll@{}}
\CodeBefore 
   % \rowcolors{2}{gray!20}{white}
\Body
\toprule
\textbf{Variable}                                          & \textbf{Definition}                                                                                                                                                              & \textbf{Scale}                                                                                                                                                                                    \\ \midrule
\multicolumn{3}{l}{\textbf{Cognitive Load Variables} \cite{CognitiveLoadTheoryFormatInstruction,Workingmemorylimitedimprovingknowledge, CognitiveArchitectureInstructionalDesign}}                                                                                                                                                                                                                                                                                                                                                                                             \\ \midrule
\begin{tabular}[t]{@{}l@{}}Intrinsic \\ load\end{tabular}  & \begin{tabular}[t]{@{}l@{}}The inherent level of difficulty \\ associated with a specific \\ topic or context\end{tabular}                                                    & \begin{tabular}[t]{@{}l@{}}How difficult is the information covered\\ in the explanations overall for you \\ to understand?\end{tabular}                                                          \\[3em]
\begin{tabular}[t]
{@{}l@{}}Extraneous \\ load\end{tabular} & \begin{tabular}[t]{@{}l@{}}Ineffective load by the manner in \\ which information is presented \\ to individuals and is under the control \\ of material\end{tabular} & \begin{tabular}[t]{@{}l@{}}How difficult is each explanation for you \\ to distinguish important and unimportant \\ information for your decision-making from \\ these explanations?\end{tabular} \\[4em]
\begin{tabular}[t]{@{}l@{}}Germane \\ load\end{tabular}    & \begin{tabular}[t]{@{}l@{}}Effective cognitive load devoted to \\ integrating new information, the \\ creation and modification of schema\end{tabular}                           & \begin{tabular}[t]{@{}l@{}}How did each explanation enhance your \\ understanding of why you were given the decision?\end{tabular}                                                             \\ \midrule
\multicolumn{3}{l}{\textbf{Decision Style Variables } \cite{DecisionMakingStyleDevelopmentAssessmentNew}}                                                                                                                                                                                                                                                                                                                                                                                             \\ \midrule
Rational                                                   & \begin{tabular}[t]{@{}l@{}}A thorough search for and \\ logical evaluation of alternatives\end{tabular}                                                                          & \begin{tabular}[t]{@{}l@{}}I make decisions in a logical and systematic way\end{tabular}                                                                                                       \\[1.5em]
Intuitive                                                  & A reliance on hunches and feelings                                                                                                                                               & \begin{tabular}[t]{@{}l@{}}When I make decisions, I tend to rely on my intuition\end{tabular}                                                                                                  \\[0.75em]
Avoidant                                                   & An attempt to avoid decision making                                                                                                                                              & \begin{tabular}[t]{@{}l@{}}I avoid making important decisions until the pressure\\ is on\end{tabular}                                                                                            \\[1.5em]
Dependent                                                  & \begin{tabular}[t]{@{}l@{}}A search for advice and \\ direction from others\end{tabular}                                                                                         & \begin{tabular}[t]{@{}l@{}}I rarely make important decisions without consulting \\ other people\end{tabular}                                                                                      \\[1.5em]
Spontaneous                                                & \begin{tabular}[t]{@{}l@{}}A sense of immediacy and a desire \\ to get through the decision-making \\ process as soon as possible\end{tabular}                                   & I generally make snap decisions                                                                                                                                                                   \\ \midrule
\multicolumn{3}{l}{\textbf{Motivation-Opportunities-Ability (MOA) model} \cite{EnhancingMeasuringConsumersMotivationOpportunity}}                                                                                                                   \\ \midrule
Motivation                                                 & \begin{tabular}[t]{@{}l@{}}Conscious and unconscious \\ cognitive processes that \\ directand inspire behavior\end{tabular}                                                      & \begin{tabular}[t]{@{}l@{}}I feel it is necessary for me to deliberately think and \\ investigate the rationale behind the decision.\end{tabular}                                              \\[2.75em]
Opportunity                                                & \begin{tabular}[t]{@{}l@{}}External factors that \\ make a behavior possible\end{tabular}                                                                                        & \begin{tabular}[t]{@{}l@{}}I feel I have enough time to deliberately think and \\ investigate the rationale behind the decision.\end{tabular}                                                  \\[1.5em]
Ability                                                    & \begin{tabular}[t]{@{}l@{}}Individual’s psychological and \\ physical ability to participate\\ in an activity\end{tabular}                                                       & \begin{tabular}[t]{@{}l@{}}I feel I have the required domain knowledge to \\ understand the information regarding my status \\ used in this decision.\end{tabular}                                \\ \bottomrule
\end{NiceTabular}
\begin{tablenotes}
  \small
  \item *All variables were measured using 5-point Likert scale.
\end{tablenotes}
\vspace{-1em}
\end{table*}
